Dissecting Distribution Inference

A distribution inference attack aims to infer statistical properties of data used to train machine learning models. These attacks are sometimes surprisingly potent, but the factors that impact distribution inference risk are not well understood and demonstrated attacks often rely on strong and unrealistic assumptions such as full knowledge of training environments even in supposedly black-box threat scenarios. To improve understanding of distribution inference risks, we develop a new black-box attack that even outperforms the best known white-box attack in most settings. Using this new attack, we evaluate distribution inference risk while relaxing a variety of assumptions about the adversary's knowledge under black-box access, like known model architectures and label-only access. Finally, we evaluate the effectiveness of previously proposed defenses and introduce new defenses. We find that although noise-based defenses appear to be ineffective, a simple re-sampling defense can be highly effective. Code is available at https://github.com/iamgroot42/dissecting_distribution_inference

==> additional_figures.tex <==
\subsection{Additional Figures} \label{app:additional_figs}

==> extra_experiments.tex <==
e)
% \begin{enumerate}
%     \item 5 models per dist: 0.7
%     \item 10 models per dist: 1.3
%     \item 25 models per dist: 1.7
% \end{enumerate}

\subsection{\amc: Ablation Study} \label{app:amc_ablation}
\anote{Probably don't need to show too many, since this attack doesn't perform that great}

\subsubsection{Using Fewer Seed Data}
\censusn\ (Gender)
\begin{enumerate}
    \item 30: 1.3 
    \item 40: 2.0
    \item 50: 2.0
\end{enumerate}

\subsubsection{Using Fewer Edges}

\subsubsection{Using Layer-Wise Models}

\subsubsection{Using Fewer Models for Training}
\censusn\ (Gender)
\begin{enumerate}
    \item 100 (80 train, 20 val): 1.5
    \item 200 (170 train, 30 val) : 2.4
    \item 400 (350 train, 50 val) : 1.6
    \item 800 (750 train, 50 val) : 2.0
\end{enumerate}

\begin{figure}[!h]
\centering
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/appendix_misc/aga_varying_models_train_box.pdf}
    \caption{Varying number of models per distribution}
    \label{fig:amc_num_models_train}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/appendix_misc/aga_varying_num_samples_box.pdf}
    \caption{Varying number of samples used}
    \label{fig:amc_num_models_train}
\end{subfigure}
\caption{...}
\label{fig:amc_variations}
\end{figure}


\subsection{\pptt: Ablation Study} \label{app:pptt_ablation}

\anote{Yifu would probably know all the variations we tried for this one}

\subsubsection{Ordering Data-Points}
The attack utilizes a heuristic (Equation~\ref{eq:pptt_ordering}) to order datapoints according to their utility, and then proceeds to select a fraction of the ordered data for the attack. To understand the impact of this ordering, ...

\subsubsection{Predictions v/s Loss Values}
Currently, the attack utilizes model predictions to compute thresholds and generate predictions. However, there is potentially additional information in labels for these samples which an adversary may be able to utilize. To explore this potential, we experimented with a variant that uses loss values instead of direct model predictions.

\subsection{\kldtest: Ablation Study} \label{app:kld_ablation}

\subsubsection{Fraction}
Since the number of possible pairwise comparisons for $n$ models grows with ${n \choose 2}$, our current attack comprises of randomly sampling a fraction of all possible pairs for use in the attack. Such a step helps combat overfitting by not utilizing \textbf{all} pair-wise comparisons (which may include patterns specific to adversary's local models), and also reduces computational complexity. For our experiments we set this ratio to be $0.8$, but did additional experiment with other ratios as well.

\boneage\ (Age)
\begin{enumerate}
    \item Ratio 0.1: 9.8
    \item Ratio 0.2: 8.9
    \item Ratio 0.5: 10.9
    \item Ratio 0.8: 22.8
\end{enumerate}

\celeba\ (Male) \fixnum{Stale}
\begin{enumerate}
    \item Ratio 0.1: 2.6
    \item Ratio 0.2: 1.7
    \item Ratio 0.5: 2.5
    \item Ratio 0.8: 3.0
\end{enumerate}

\censusn\ (Gender) \fixnum{Stale}
\begin{enumerate}
    \item Ratio 0.1: 8.8
    \item Ratio 0.2: 8.9
    \item Ratio 0.5: 8.8
    \item Ratio 0.8: 7.9
\end{enumerate}

\subsubsection{Voting}
Equation~(\ref{eq:weight_vote}) computes a ``weighted vote" from all of the adversary's models. For our initial attack design, we implemented the simple variant where instead of weighted votes, each comparison yields a binary 0/1 prediction. These predictions are then aggregated to generate the final prediction $\hat{b}$. We term this other variant ``simple vote".  

\subsection{Identifying Useful Layers}

As explored by Suri et. al.~\cite{suri2022formalizing}, different layers of the model capture information pertinent to the property differently. An adversary may thus want to carefully pick layers of the victim's models to target. Although this is not possible in black-box attacks, it can be achieved in the white-box access setting by using intermediate feature activations from only certain layers for the \amc. Instead of trying meta-classifiers for all layers, we chose to identify layers with the most unique feature activation patterns. This can help reduce parameters in the meta-classifier, and potentially improve attack performance.
To identify useful layers, we utilize the Centred Kernel Alignment (CKA) method~\cite{kornblith2019similarity} to inspect layer-wise feature activations from models. This analysis helps identify 'groups' of layers with similar activation patterns. An example is shown in Figure~\ref{fig:cka_analysis} for \celeba\ (Age): the last three layers (linear) form a group very different from the first five layers (convolutional), as apparent in the similarity values.

\begin{figure}[!h]
\centering
\begin{subfigure}[b]{0.241\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/appendix_misc/cka_experiment_celeba.png}
    \caption{CKA Analysis for \celeba\ (Young)}
    \label{fig:cka_analysis}
\end{subfigure}
% \hfill
% \begin{subfigure}[b]{0.241\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/celeba/kl_all_box.pdf}
%     \caption{\kldtest}
%     \label{fig:celeba_kl_all}
% \end{subfigure}
\caption{...}
% \label{fig:celeba_task_prop_pairs}
\end{figure}

We evaluate this experiment for \celeba\ (Age), using 15 models per distribution to estimate CKA values. Concretely, we utilize the second and third convolutional layers, along with the last two fully-connected layers. We observe a slight increase in performance-- \neff\ increases slightly from $0.8$ to $0.9$. There does seem to be scope in improving performance of white-box attacks using such layer identification and selection methods. However, given the superior performance of black-box attacks in our experiments, we leave this exploration as part of future work.

==> interpret.tex <==
\section{Interpretability} \label{sec:interpret}

White-box attacks, which utilize meta-classifiers and are usually the most performant attacks against distribution inference, utilize model parameters in a complicated way. Recognizing patterns across models and how they differ across training distributions can help both adversaries and victims alike---designing better attacks, and understanding inference risks for the models they release, respectively. While interpreting the features learned by the Permutation Invariant Network is understandably hard, our proposed \amc\ can be studied to better understand the kind of signals it utilizes to distinguish between models with different training distributions.

We use Integrated Gradients~\cite{sundararajan2017axiomatic} to assign importance scores to input features which, in the case of \amc, are pair-wise cosine similarity scores across all layers. We aggregate importance scores across layers, giving us mean feature importance scores for each pair of datapoints. After selecting a subset of these features (different cases discussed in ...), we backtrack the pairs and identify individual points which the pairs correspond to.

Since the idea of distribution inference is to look at dataset-wise properties, we decide to look at data in groups--- we look at the model's predictions for each pair of datapoints, and then visualise these points on a simple 2D graph, with edges between all pairs of points.

\begin{figure*}[!h]
\centering
\begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/interpretability/Interpret_all.png}
         \caption{All Features}
         \label{fig:interpret_all}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/interpretability/Interpret_top.png}
         \caption{Top 5\% Features}
         \label{fig:interpret_top_five}
\end{subfigure}
\caption{Datapoints corresponding to features used for the \amc\ for  (\subref{fig:interpret_all}) all features and top 5\% features (\subref{fig:interpret_top_five}), for \celeba. Orange points have a predicted task label of 0, while blue points have a predicted task label of 1. Edges between points exist for pairs that are used by the \amc. As visible, several edges share points. (Will update will improved figures later- placeholder for now)}
\label{fig:interpret}
\end{figure*}

\shortsection{Edges with Anchor Nodes}

\shortsection{Edges with Similar Predictions}

\shortsection{Edges with Different Predictions}
